Online Nash Social Welfare Maximization with Predictions

We consider the problem of allocating a set of divisible goods to $N$ agents in an online manner, aiming to maximize the Nash social welfare, a widely studied objective which provides a balance between fairness and efficiency. The goods arrive in a sequence of $T$ periods and the value of each agent for a good is adversarially chosen when the good arrives. We first observe that no online algorithm can achieve a competitive ratio better than the trivial $O(N)$, unless it is given additional information about the agents' values. Then, in line with the emerging area of "algorithms with predictions", we consider a setting where for each agent, the online algorithm is only given a prediction of her monopolist utility, i.e., her utility if all goods were given to her alone (corresponding to the sum of her values over the $T$ periods). Our main result is an online algorithm whose competitive ratio is parameterized by the multiplicative errors in these predictions. The algorithm achieves a competitive ratio of $O(\log N)$ and $O(\log T)$ if the predictions are perfectly accurate. Moreover, the competitive ratio degrades smoothly with the errors in the predictions, and is surprisingly robust: the logarithmic competitive ratio holds even if the predictions are very inaccurate. We complement this positive result by showing that our bounds are essentially tight: no online algorithm, even if provided with perfectly accurate predictions, can achieve a competitive ratio of $O(\log^{1-\epsilon} N)$ or $O(\log^{1-\epsilon} T)$ for any constant $\epsilon>0$.

==> additional_related.tex <==
\citet{GPT21} study the extent to which online algorithms can maximize the utilitarian social welfare, while satisfying envy-freeness. They make the simplifying assumption that the sum of every agent's valuations are normalized to 1, i.e., that $V_i=1$ for all $i$. This is a significantly more stringent assumption than the one that we make in this paper, where $V_i$ can take any value and we require only a rough estimate to achieve our bounds. However, even with this assumption, they show that the best possible approximation for instances with $n$ agents is $O(\sqrt{n})$, so they focus on designing mechanisms for instances with just two agents. 

%The same issues arise even for very different notions of fairness than the ones considered in this paper. 
\citet{BKPP18} consider a setting similar to ours, but the items being allocated in their case are indivisible, i.e., can be allocated only to a single agent (so they use randomness). Their goal is to minimize the amount of envy among the agents, and they show that the best way to minimize the expected maximum envy (up to sub-logarithmic factors) is to totally disregard the agent valuations and allocate each item uniformly at random among the agents, leading to a bound of $\tilde O(\sqrt{T/N})$. 
% \citet{BKPP18} consider a setting where a set of items arrive in a sequence of $T$ rounds, and an algorithm needs to allocate them in an online manner. The main differences to our work is that they focus on items that are indivisible, i.e., can be allocated only to a single agent, and that they use the amount of envy among the agents as a measure of fairness. 
%\citet{BKPP18} show that allocating each item uniformly at random among the agents, without taking their values into consideration, leads to an expected maximum envy among the agents of $\tilde O(\sqrt{T/N})$ and they argue that this bound it tight up to polylogarithmic factors. They then also propose a more elaborate deterministic algorithm that depends on the agent values and achieves the same bound. 
%
\citet{ZP20} revisit this setting and study the extent to which approximate envy-freeness can be combined with approximate Pareto efficiency. They consider a spectrum of increasingly powerful adversary models and they show that even for a non-adaptive adversary (which is weaker than the adaptive adversary model we consider in this work) there is no algorithm that can guarantee the aforementioned approximate envy while Pareto dominating the random allocation algorithm. They define an outcome to be $\alpha$ Pareto-efficient if improving every agent's utility by a factor $\alpha$ is infeasible, and they show that it is impossible to combine the envy bound with a $1/N$ approximation of Pareto efficiency, which is a trivial approximation that the random allocation algorithm satisfies. Note that our competitive ratio guarantees in this paper directly translate into approximate Pareto efficiency bounds. Specifically a competitive ratio of $\alpha$ for the the Nash social welfare directly implies an $\alpha$ approximation of Pareto efficiency.
%
%One way to interpret this is that sublinear envy is a very strong fairness constraint, and it does not allow for non-trivial Pareto-optimality guarantees (as $1/n$ factor can be achieved by just splitting each item equally across the agents). 

%Although some of the obstacles that we face in this paper are similar, in essence, to the ones that this prior work aims to address, our results are not directly comparable. In particular, we evaluate the quality of the outcomes using aggregate measures of fairness instead of pairwise fairness, so our bounds do not directly translate into interesting guarantees for envy-freeness, or vice-versa. On the other hand, our competitive ratio guarantees do directly translate into approximate Pareto efficiency bounds. In particular a competitive ratio of $\alpha$ for the maxmin welfare or the Nash social welfare directly implies an $\alpha$ approximation of Pareto efficiency. 


\citet{BMS19} also consider the sequential allocation of divisible resources, and they impose a normalization on the agent valuations similar to the one in \cite{GPT21}. The main differences are that they enforce envy-freeness as a constraint, and instead aim to maximize social welfare, and, more importantly, that they assume the valuation vectors of the agents are drawn from a distribution. Using this assumption, they weaken the fairness envy-freeness constraint to be satisfied only in expectation.
\citet{HPPZ2019} also study a similar setting, but allow the reallocation of some of the previously allocated items, and show that envy-freeness up to one item can be achieved using $O(T)$ re-allocations. Other works consider the question of online fair division with random agent valuations, e.g. \citet{sinclair2020sequential} look at envy-freeness and efficiency with respect to the hindsight optimal solution, while
%\citet{BMS19} consider objectives of fair-share and welfare, 
%\citet{ZP19} concentrate on envy-freeness and Pareto-optimality, and 
\citet{KPW16} study the maxmin share in such a setting. Another line of work on dynamic fair division, which is not very closely related to our work, considers settings where it is the agents, instead of the items, that arrive (and possibly depart) online, e.g., \cite{FPV17,FPS15,LLY18}.

==> obstacles.tex <==


The main idea behind this proof is one that also provides some intuition for the much more demanding lower bound construction of~\cref{sec:hardnessNSW}. In particular, when facing an instance where the agents appear similar during the first rounds, an online algorithm cannot do better than treating them in a symmetric fashion. However, some of these agents may later on have a high value during a round with low competition, and are therefore easy to satisfy, while others may only value items during rounds with high competition, which makes them hard to satisfy. An algorithm with access to future valuations would therefore prioritize the latter agents during the first rounds, making the optimal solution significantly better than what any online algorithm can hope to achieve. 

\begin{theorem}
\label{thm:impossibility_maxmin}
For the objective of maxmin welfare, there is no online algorithm that can guarantee a competitive ratio better than $\frac{\sqrt{N}}{3}$, nor is there an online algorithm that can guarantee a competitive ratio better than $\frac{\sqrt{T}}{3}$. 
\end{theorem} 
\begin{proof}
To prove the desired bounds on the competitive ratio of any given online algorithm, we construct an instance adaptively depending on the decisions of the algorithm. Without loss of generality, we assume that $N$ is even and that $\sqrt{N}$ is an integer. In the first round of this instance, the valuation of every agent $i$ is equal to $v_{i,1} = 1-\frac{1}{\sqrt{N}}$. 

Irrespective of how the online algorithm allocates the item of the first round, the number of agents that receive at least a $2/N$ fraction of the good in this round is at most $N/2$ (since these fractions add up to at most 1), which implies that at least $N/2$ agents receive less than a $2/N$ fraction. Let $A$ be a subset of any $\sqrt{N}$ of these agents, who receive less than $2/N$ of the item and hence obtain less than $2/N$  utility from it. Without loss of generality, we assume that agents in $A$ are the last in the ordering: $A = \{i\in[N]: i>N-\sqrt{N}\}$.

In each of the next $N-\sqrt{N}$ rounds, the item is valued only by a single distinct agent not in $A$ for a value of $v_{i,i+1} = \frac{1}{\sqrt{N}}$ (i.e., all of the remaining value of that agent), and all other agents have a value of zero for it: $v_{i,t}=0$ if $t\neq i+1$. Finally, in the last round all the agents in $A$ have a value of $1/\sqrt{N}$ for the same item $v_{it} = \frac{1}{\sqrt{N}}$.

One feasible allocation for this instance would be to allocate the items of the first and last round equally among the $\sqrt{N}$ agents in $A$, providing them with a utility of $\frac{1}{\sqrt{N}}$ each, and then allocating each of the remaining items fully to the distinct agent that values them, providing the remaining agents with a value of $\frac{1}{\sqrt{N}}$ as well. Therefore, the optimal maxmin welfare is at least $\frac{1}{\sqrt{N}}$.

On the other hand, since the outcome of the online algorithm allocated no more than a $2/N$ fraction of the first item to each of the agents in $A$, the average value these agents receive from the first and the last item is no more than $\frac{2}{N}\left(1-\frac{1}{\sqrt{N}}\right)+\frac{1}{\sqrt{N}} \frac{1}{\sqrt{N}}\leq \frac{3}{N}$. Since the minimum value among the agents in $A$ is less or equal to their average value, we conclude that the competitive ratio of the algorithm is at least $(1/\sqrt{N})/(3/N)=\sqrt{N}/3$.

Since the family of instances described above has a total number of rounds $T=N-\sqrt{N}+2$, this directly implies that no online algorithm can guarantee a competitive ratio better than $\sqrt{T}/3$ for all values of $T$.
\end{proof}

Note that this proof employs the adaptive adversary model, that is, the adversary's choices for future rounds depend on what the online algorithm does on the current round. However, for deterministic algorithms this is equivalent to a static adversary (one who chooses the entire instance in advance). This difference in adversary model only plays a role for randomized algorithms, but in the setting of divisible items we consider here any randomized algorithm can be converted into a deterministic one with the same competitive ratio \footnote{Here we assume that competitive ratio for a randomized algorithm is measured using the same metric (e.g., maxmin welfare) applied to expected utilities of agents.}.

In contrast to the negative result of this section for the maxmin welfare, the next section considers the Nash social welfare objective and provides an online algorithm that guarantees a logarithmic competitive ratio with respect to both $n$ and $T$. \Cref{sec:hardnessNSW} then shows that this is the best competitive ratio that any online algorithm can achieve.

% \section{Obstacles to Fairness in Online Allocation}
% \label{sec:lowerbounds}

% \begin{lemma}
% No algorithm can achieve a NSW approximation better than $e^{1/e} \sim 1.45$
% \end{lemma}

% \begin{proof}
% Fix a constant $\beta \in (0,1)$. Consider the following instance. There are $\beta N$ agents we will call "clashing" and $N-\beta N$ "resolving" agents (the intuition for naming will become apparent in the following description).

% On $t=1$ every agent has value $1-\frac{1}{\beta N}$.

% On $t=2$ all clashing agents all have value $\frac{1}{\beta N}$ and all resolved agents have value $0$. 

% For remaining turns $t = 3\ldots N-\beta N+2$ one of resolving agents has value $\frac{1}{\beta N}$ and everyone else has value zero on each period.

% The intuition for this example is that no algorithm will be able to differentiate between clashing and resolving agents on the first period and cannot do better than to distribute the good equally, while the optimal policy allocates the good to clashing agents (as they won't be able to derive much value later) and doesn't allocate to resolved agents (since they'll get their share later)
% \end{proof}

% Formally, distributing the good only between clashing agents for $t=1,2$ and allocating the good to the corresponding resolving agent on remaining turns yields

% $$NSW^* = \left [ \left (\frac{1}{\beta N} \right )^{\beta N} \left( 1-\frac{1}{\beta N}\right)^{1-\beta N}\right ]^{1/N}$$

% Meanwhile, distributing the good equally between everyone on $t=1$, and doing the same allocation on the remaining turns (and no myopic policy can do better than this) yields

% $$NSW^{greedy} \leq \left[ \left (\frac{1}{N}+\frac{1}{(\beta N)^2} \right )^{\beta N} \left( 1-\frac{1}{\beta N}+\frac{1}{N} \right)^{1-\beta N} \right ]^{1/N}$$

% For large $N$ (keeping $\beta$ fixed) this gives

% $$
% \frac{NSW^{greedy}}{NSW^*} \leq \beta^\beta
% $$

% Optimizing this ratio over $\beta$ gives the desired lower bound.
